Extreme Masking for Learning Instance and Distributed Visual Representations

The paper presents a scalable approach for learning spatially distributed visual representations over individual tokens and a holistic instance representation simultaneously. We use self-attention blocks to represent spatially distributed tokens, followed by cross-attention blocks to aggregate the holistic image instance. The core of the approach is the use of extremely large token masking (75\%-90\%) as the data augmentation for supervision. Our model, named ExtreMA, follows the plain BYOL approach where the instance representation from the unmasked subset is trained to predict that from the intact input. Instead of encouraging invariance across inputs, the model is required to capture informative variations in an image. The paper makes three contributions: 1) It presents random masking as a strong and computationally efficient data augmentation for siamese representation learning. 2) With multiple sampling per instance, extreme masking greatly speeds up learning and improves performance with more data. 3) ExtreMA obtains stronger linear probing performance than masked modeling methods, and better transfer performance than prior contrastive models.

==> intro.tex <==
\section{Introduction}

Unsupervised learning becomes the center of computer vision research in recent years. The goal of unsupervised learning is to achieve generalization which facilitates building label efficient downstream applications.
Past works demonstrate generalization through k-nearest-neighbors~\cite{wu2018unsupervised} and zero-shot classification on the learned features~\cite{radford2021learning}, or finetuning the model for a limited schedule~\cite{chen2020simple,bao2021beit}.

The approaches to achieve generalization and the understandings about the nature of generalization are developing fast.
One popular approach is to learn invariances through image transformations such as resized cropping and color jitter.
Such invariances encode useful high-level properties about the desired representations. Contrastive models~\footnote{In this paper, we broadly refer methods even without negative pairs as contrastive models, such as BYOL and DINO. } learned from heavy engineered image transformations are shown to produce high-level features that are on par with supervised learning.

An emerging trend of masked image modeling approach, however, does not rely on heavy image transformations. Given a single image crop, a large portion (up to 75\%~\cite{he2021masked}) of the image content are masked. The network is trained to predict the masked patches from the visible ones in a BERT~\cite{devlin2018bert} fashion.
Instead of finding invariances, the network has to ``memorize'' the visual content with accurate spatial, scale and color variations in a non-trivial way. Despite of lacking explicit high-level invariances, masked image modeling shows remarkable generalization performance  when finetuned for transfer learning~\cite{li2021benchmarking} especially for transformer architectures~\cite{dosovitskiy2020image}.

The distinctions between the two approaches are not limited to the pretext tasks, but also fundamentally about the way to represent data. Contrastive methods extract the global representation for an entire image, whereas masked modeling uses a distributed representation~\cite{mikolov2013distributed} over individual tokens with token-level supervision to ensure correspondence.
Given these differences, little is explored and understood about the connection between them.

%In this paper, we hope to bridge the connection for contrastive learning and masked image modeling, and advance the research for representation learning.
In this paper, we propose a novel approach that learns the distributed representation as well as the instance representation simultaneously from instance supervision alone. 
We start with an observation that random masking could be viewed as a novel scheme of data augmentation, which is never exploited for prior contrastive models. 
We then explore a simple model where the instance representation with masked input is trained to predict that from the full view, in a plain BYOL fashion~\cite{grill2020bootstrap}. We adopt visual transformer ViT~\cite{dosovitskiy2020image} to embed distributed representations over patches, and a followed class-attention blocks~\cite{touvron2021going} to aggregate  the instance representation. The instance-level learning objective supervises both the distributed and instance representations.



Our model combines the random masking procedure in masked image modeling as a novel data augmentation and the learning objective in BYOL framework. Compared with masked modeling, our model has the following advantages: 1) It uses extremely large masking ratio of 90\% (compared with 75\%~\cite{he2021masked}) for best performance and computational efficiency. This allows multiple masked inputs with marginal computation overhead. 2) The instance representation from our model could be used off-the-shelf for measuring semantic similarities. 3) The framework welcomes other data augmentations besides masking, such as scaling, translation and color jittering for multiple views. 

Compared with typical contrastive learning models~\cite{chen2020simple,caron2021emerging,chen2021empirical}, our model does not rely on data augmentation induced invariances to achieve generalization. 
%It is not encouraged to learn invariances through traditional image augmentations.
Rather, our model preserves all possible useful variations from the masked view in order to recover the full. We give demonstrations of the generative aspects of our model in Figure~\ref{}. It can faithfully inpaint the masked pixels through network inversion~\cite{zhao2020makes}. This shows that the model learns a distributed representation that well captures scale, location, and color intensities.

We apply the model on ImageNet-1k for representation learning and evaluate its transfer performance on image classification, semi-supervised learning, and semantic segmentation. We evaluate image classification using both linear probe on the instance representation and end-to-end finetuning on the distributed representations. Our model achieves similar finetuning results with masked modeling approaches, while outperforming them with linear probe by a large margin. We ablate the role of data augmentation induced invariances in our framework, finding that invariances may improve the instance representation, but being detrimental to the distributed representations especially for dense prediction applications which requires detailed spatial reasoning. 




figures in the paper: 
overview, reconstruction, knn for instance, attention, 

Zhirong: Not sure if it is proper to use the word "contrastive" in the paper
\steve{Since BYOL distinguishes itself from contrastive approaches, it seems that a different name is needed here, though I'm not sure what. Have these recent methods without negatives used a name for their general approach?}

\steve{We should find something to say about why random masking causes contrastive models to behave so differently than with other augmentations. To me, this is what the introduction ideally should focus on. Conventional augmentations in contrastive learning could be viewed as delineating an appearance subspace for a given class. All of the augmented views are valid appearances of the class, and contrastive models seek a single representation vector that encompasses this subspace. Can it be said that random masking enables this to happen in a much more general and powerful way? Rather than offering very narrow self-supervision (e.g., that two conventionally augmented images belong to the same class), random masking allows any image that is consistent with the masked image to belong to the same class as the unmasked image. This self-supervision goes well beyond what can be described by conventional augmentations, as the potential degrees of freedom within the masked areas are innumerable. Yet these masked areas seem not to be fully unconstrained, since the distributed representations that you've found roughly approximate the unmasked image. Perhaps the contrastive loss over many training pairs will encourage representation of geometric structure like in MAE? Anyway, please let me know your thoughts on this.} \xiao{One viewpoint that differentiates random masking from other augmentations (random crop, basically) is its ability to maintain a large receptive field under extreme masking. First, let's say extreme masking could facilitate representation learning (an insightful explanation is needed though, for example, 1. it forces the network to learn richer part-whole dependencies; 2. the intrinsic characteristics of an object class are encoded in the network rather than leaking out from partial observations.). Then, random masking actually keeps the original image’s receptive field, where the correlation between reserved pixels and masked pixels would be much closer and richer, compared to random cropping.}
\steve{Why this approach is able to model the full receptive field is a critical question. It is puzzling to me that it does this without explicit guidance like a reconstruction loss. Given that the supervision is only at the instance level, I would have guessed the representation to model only what the two images have in common (the unmasked areas) without considering the rest, but apparently this is not the case. Do any of you have thoughts on this? I have a feeling that the improvement with greater masking is revealing something important about the underlying mechanism. Are there other results that might also shed some light?}
\steve{Maybe this behavior follows from Zhirong's previous observation that instance discrimination tends to preserve as much information as possible, in order to make an instance more unique from other instances? If this is the case, then this approach may favor a representation that comprehensively models the original image and learns to map the masked image to this representation. But should this information preservation property still hold when training without negatives, as there is no constraint towards improving discrimination?}
\xiao{I've learned more from Zhirong’s technical details in Section 3. The momentum encoder processes the full image crop (unmasked) $\mathbf{I}$, while the base encoder processes the greatly masked version of $\mathbf{I}$, termed $\mathbf{U}$. Then the learning objective is to recover the masked regions ($\mathbf{I} - \mathbf{U}$) from $\mathbf{U}$ in the feature space. This objective looks more like a reconstruction loss (of the greatly masked regions $\mathbf{I} - \mathbf{U}$) in the feature space, than only modeling what the two images have in common at the instance level.}
\xiao{Forcing a small part of an image to recover the full image encourages the network to almost remember the entire object class, as well as rich dependencies between part and whole, I guess. Then, I can imagine how this is done even without negatives by considering the learning process as a clustering process of all small parts of an object class. Those small parts are collected, not only from different crops and masks of the same image, but also potentially from other images of the same object class since their small parts should have a lot in common.}
\steve{Does the model require multiple various parts of the same image or similar images for training? Is this the key to learn full-image reconstruction or can the model still learn this without such data?}\xiao{I guess there are two possible ways to make an image ($\mathbf{I}$) and a part of it ($\mathbf{U}$) to have the same instance representation. One way is to degenerate $\mathbf{I}$ into $\mathbf{U}$, and the other way is to complete $\mathbf{U}$ into $\mathbf{I}$ instead (the reconstruction is done in the sense of this completion). Maybe some mechanism is preventing the first case from happening? For example, $\mathbf{I}$ is required to have the same representation with multiple various parts of $\mathbf{I}$.}\xiao{Just to be sure, $\mathbf{U}_1$ and $\mathbf{U}_2$ are two different parts of $\mathbf{I}$, the model requires not only $\mathbf{U}_1$ and $\mathbf{I}$ to have the same representation, but also $\mathbf{U}_2$ and $\mathbf{I}$ to have the same representation.}
\steve{I mean, does the model require $\mathbf{I}$ and multiple of its $\mathbf{U}$ for training, otherwise it will not learn full-image reconstruction? Or will it learn it even if given only a single $\mathbf{U}$? I wonder about the role of the training data.}\xiao{Yes, the model require $\mathbf{I}$ and multiple of its $\mathbf{U}$ for training, there are many ($\mathbf{I}$, $\mathbf{U}_n$) pairs trained.}
\steve{So it won't work otherwise? I just want to make sure that we are certain about this explanation.}\xiao{Sorry I don't know if it works otherwise or not. Maybe Zhirong has some experiment results} \steve{If there is some experimental support for this explanation, that would be great to show. It makes sense, but I am not 100\% sure.}\xiao{Yes, an experimental support would help the explanation, but I'm not sure this is the right answer either.} \steve{Maybe a different reason for learning full-image reconstruction is because the initial model will produce a full-image representation in the teacher branch, so the student branch will generally be encouraged to do so as well.} \xiao{Yes I think so. In addition, the teacher branch is actually never trained, the gradient is blocked in the teacher network. It is the student network that has been training throughout the training process, and the learning objective of the student network is always to let U approach I.} \steve{Yes, it would be good to get more certainty about the underlying reasons for why the model is successful for full-image reconstruction.} \xiao{Yes. I wonder if the network never got a change to learn how to degenerate I into U since gradient is always blocked in the teacher branch, then maybe a single U would also work.}
\iffalse

Entangled invariances.

Results?

Masked image modeling and random masking operations.

discriminative models vs generative models.

the connection between MIM and contrastive learning.

skip-gram

fixmatch , weak and strong augmentations

invariances and generalization

Distributed representation and global reprentation

\fi
